ClearMark: Intuitive and Robust Model Watermarking via Transposed Model Training

Due to costly efforts during data acquisition and model training, Deep Neural Networks (DNNs) belong to the intellectual property of the model creator. Hence, unauthorized use, theft, or modification may lead to legal repercussions. Existing DNN watermarking methods for ownership proof are often non-intuitive, embed human-invisible marks, require trust in algorithmic assessment that lacks human-understandable attributes, and rely on rigid thresholds, making it susceptible to failure in cases of partial watermark erasure. This paper introduces ClearMark, the first DNN watermarking method designed for intuitive human assessment. ClearMark embeds visible watermarks, enabling human decision-making without rigid value thresholds while allowing technology-assisted evaluations. ClearMark defines a transposed model architecture allowing to use of the model in a backward fashion to interwove the watermark with the main task within all model parameters. Compared to existing watermarking methods, ClearMark produces visual watermarks that are easy for humans to understand without requiring complex verification algorithms or strict thresholds. The watermark is embedded within all model parameters and entangled with the main task, exhibiting superior robustness. It shows an 8,544-bit watermark capacity comparable to the strongest existing work. Crucially, ClearMark's effectiveness is model and dataset-agnostic, and resilient against adversarial model manipulations, as demonstrated in a comprehensive study performed with four datasets and seven architectures.

==> 98_acknowledgement.tex <==
%-------------------------------------------------------------------------------
\section*{Acknowledgments}
%-------------------------------------------------------------------------------

TODO Acknowledgement

==> approach_tmp.tex <==
\commentA{The following text until the end of the paragraph does not explain the method but rather lists its benefits. I would move this discussion to be after "Principle of TCPmark", as one would better understand why these properties hold}
  \ournameGen verification process yields an input-like sample that resembles the secret, e.g., an image, which can be intuitively analyzed through visual inspection by humans and machines. 
 %This makes the copyright infringement decision-making process more human-understandable and intuitive, which is a criterion that strengthens argumentation about copyright claims in front of non-tech-savvy people, e.g., in court cases. 
\ourname is the first method to leverage \textit{transposed model functionality} (\cf~\hyperref[sec:background:transposed]{\sect\ref{sec:background:transposed}}) for embedding the watermark, essentially filling unused model capability. The entanglement of the watermark with all parameters increases the watermark's robustness, e.g., against fine-tuning, and capacity, and enforces significant sacrifices in model performance if the watermark is removed. %As the watermark gets intertwined with the model's main task, it resists potential malicious changes to the model, e.g., fine-tuning, or its removal, which simultaneously negatively affects the model's main task. 

==> info_two_losses.tex <==
When you want to optimize a set of parameters with respect to two loss functions, you are essentially dealing with a multi-objective optimization problem. There are several methods you can consider for optimizing parameters in this scenario:

1. **Weighted Sum Method:** In this approach, you combine the two loss functions into a single composite loss function by assigning weights to each loss. The combined loss is then optimized using a standard optimization algorithm. The choice of weights determines the trade-off between the two objectives. This method simplifies the problem into a single-objective optimization but may require tuning of the weights.

2. **Pareto-Based Methods:** Instead of combining the losses, you can aim to find a set of parameters that represent a Pareto-optimal solution, where no further improvement in one objective can be achieved without degrading the other. Multi-objective optimization algorithms, such as NSGA-II (Non-dominated Sorting Genetic Algorithm II) or MOGA (Multi-Objective Genetic Algorithm), can help you find the Pareto front, which is a set of solutions that represent trade-offs between the objectives.

3. **Sequential Optimization:** You can optimize the parameters sequentially for each loss function, fixing the parameters optimized in the previous step. This approach alternates between optimizing for one loss and then the other. It may require multiple iterations to reach convergence.

4. **Constraint Optimization:** Treat one loss function as the primary objective and the other as a constraint. You aim to minimize the primary loss while satisfying constraints imposed by the secondary loss. Constraint optimization methods like the Alternating Direction Method of Multipliers (ADMM) can be used for this purpose.

5. **Hybrid Methods:** You can also explore hybrid methods that combine elements of the above approaches. For example, you might use a weighted sum method with an additional constraint to ensure that one loss doesn't degrade beyond a certain threshold.

The choice of method depends on the specific characteristics of your problem, the nature of the two loss functions, and your objectives. Each method has its strengths and weaknesses, and the most suitable one for your problem may require experimentation and testing. Additionally, the choice of method may impact the interpretability and robustness of your model, so consider these factors as well when making your decision.




Sequential method:
Here's how it works:

1. **Optimize for the First Loss:** In the first step, you optimize the model parameters to minimize the first loss function while keeping the second loss function constant. This means that you focus solely on minimizing the first loss, treating it as the primary objective.

2. **Optimize for the Second Loss:** In the second step, you fix the parameters obtained from the first step and optimize the model parameters to minimize the second loss function while keeping the first loss function constant. Now, you focus on minimizing the second loss, treating it as the primary objective in this step.

3. **Repeat as Needed:** Depending on your goals, you can repeat these steps as many times as necessary, alternating between optimizing for each loss function. This process continues until you achieve a satisfactory solution or convergence.

Sequential optimization is a simple and intuitive approach to handle multi-objective optimization problems when you have two conflicting objectives (represented by the two loss functions). However, it may require multiple iterations to reach a good solution, and there is no guarantee of finding a globally optimal solution.

This method can be effective for certain problems but may not be as efficient or principled as more advanced multi-objective optimization techniques, such as Pareto-based methods or constraint optimization, especially if the trade-offs between the objectives are complex or if you have specific constraints to satisfy. The choice of optimization method should be based on the characteristics of your problem and your optimization goals.

==> intro_my_content.tex <==
Machine Learning is a raising technology, that has a lot of advanatages, mainly automation of processes decission and recommendation making based on historical data. The technology is already used in real life e.g. in image classification, e.g. for medical image analysis, natural language processing, e.g. text prediction, as well as other domains, like autonomous driving, or translation. Central part of a machine learning system is the model, e.g. a DNN,  and on the other side the data. Especially the second, the data, are often hard and difficult to aquire such that huge costs are involved, might be sensitive, e.g. in the case of medical images, or belong to the intellectual Property (IP) of the model creator. As soon as data are available, computational resources need to be leveraged to train the model, which of course also takes effort and hence produces costs. Hence, the resulting trained model can also be considered IP of the model creator. 

As soon as the model is made publicly available or sold to third parties, the question of digital rights managment arrises. When considering adversarial parties, such a model can be either stolen but also reselled, modified, or illegimatelly used without respective license. Such scenarios called copyright infringements are liable to prosecution / can be sued in court.

For classical media, like images or audio, it is common practice to embedd a visible or unvisible so called watermark onto the media, which allows ownership proof. In the case of an image, such a watermark could be a stamp on the image, such that removing the watermark without making the image useless is not possible. The same principle can be applied when it comes to machine learning models.

Existing DNN watermarking methods mostly consist of a key as input to an algorithm that extracts the watermark from the model, which produces an output, which is then verified against the ground truth secret of the watermark. The different watermarking can be mainly categorized with respect to two different properties. They can be white-box or black-box, depending on if the watermark can be extracted only with direct access to the model or by only requesting predictions on the model e.g. via an API. The DNN watermarking methods can be 1-bit or multi-bit, depending on if the watermark is verified by pure existance of the watermark or if the watmermark itself contains additional information, like a name for example. 

However, all those watermarks embed human-invisible watermarks. Therefore, for watermark verification the tester needs to trust the algorithm, which usually extracts data from the DNN, which lacks in being human-understandable. This data is then reduced to one single value, which is then compared to a hard threshold, which e.g. claims watermark existance above the threshold and an invalid watermark test below the threshold. However, during watermark verifications, situations can occur, where the watermark is partly erased from the media, but a human could clearly understand and see, that the watermark was previously present and hence claim copyright infrindgement, while an algorithm categorizes the watermark as invalid as the value is slightly below the threshold. As copyright infringements must be evaluated by often non-tech-savy people, e.g. judges, the evaluation method should be intuitive and human understandable, such that a human can make the final decision. 

In this paper, we address this problem and propose TCPmark, the first multi-bit, white-box DNN watermarking method that follows an intuitive approach and embedds a visible watermark, that can be analyzed by human inspection, allowing the human to make the final decision based on sanity and reason, but could also be assisted or fully replaced by technology-based evaluation methods. Thereby, the watermark must not depend on a specific model or dataset and must withstand adversaries, that manipulate the model by continuing training on thrid party datasets or that try to remove the watermark with knowledge of the watermark method.

To address the aforementioned problems this paper makes the following contributions:

- We propose TCPmark, the first DNN watermarking mechanism with human-visible and understandable output that does not rely on a hard value threshold but on human ability to judge. This circumstance allows for more coherent and plausible jurisdiction, e.g. if only small but obvious portions of the watermark are remaining, and hence more security of the model creators' intellectual property.

- We are the first approach that uses transposed model training for emebedding a visible and human understandable watermark into a DNN. Thereby, we train the model from backwards to embedd the watermark, while regular (forward) training remains normal for the models main task.

- We entangle the watermark and the main task together within all parameters to create a robust watermark against adversarial model manipulations, e.g. fine-tuning on third party datasets, pruning of model parameters, or adaptive adversaries, that try to remove or overwrite the watermark. By our design, a malicious modification necessitates sacrifices in the main task performance of the model essentially rendering the model useless.

- We conduct a systematic large-scale study to analyze the factors that influence TCPmark and deponstarte its independence from application specific factors like dataset and model architectures. Further the watermark robustness is tested under various fine-tuning and pruning scenarios. Furhter, we provide incidence, that the capacity of TCPmark exceeds existing works with 8000 bits that can be embeded.

Overall, our work proposes a highly intuitive and easy-to-understand white-box multi-bit DNN watermarking method, with large capacity that is robust under various attack scenarios. The embedded watermark is human-understandable, addressing the weakness of existing solutions, that are complicated in design and non-intuitive especially in the final decission making process, which can be done by a human in the case of TCPmark.

